Learning Utilities and Equilibria in Non-Truthful Auctions

In non-truthful auctions, agents' utility for a strategy depends on the strategies of the opponents and also the prior distribution over their private types; the set of Bayes Nash equilibria generally has an intricate dependence on the prior. Using the First Price Auction as our main demonstrating example, we show that $\tilde O(n / \epsilon^2)$ samples from the prior with $n$ agents suffice for an algorithm to learn the interim utilities for all monotone bidding strategies. As a consequence, this number of samples suffice for learning all approximate equilibria. We give almost matching (up to polylog factors) lower bound on the sample complexity for learning utilities. We also consider a setting where agents must pay a search cost to discover their own types. Drawing on a connection between this setting and the first price auction, discovered recently by Kleinberg et al. (2016), we show that $\tilde O(n / \epsilon^2)$ samples suffice for utilities and equilibria to be estimated in a near welfare-optimal descending auction in this setting. En route, we improve the sample complexity bound, recently obtained by Guo et al. (2021), for the Pandora's Box problem, which is a classical model for sequential consumer search.

==> search-ICML.tex <==
In this section we consider auctions in which bidders do not know their values a priori and have to pay a cost to know their values.


% This model was proposed and studied by \citet{KWW16},
% who showed that a descending price auction with search costs has the same set
% of equilibrium (in terms of allocation and payments) as a first price auction
% without search cost but with the value distributions transformed; the maximum
% welfare under the transformed distribution is just the maximum welfare
% achievable under the original distributions with search costs.

% The main result of this section is that, in presence of search costs but
% unknown value distribution, $\tilde O(n / \eps^2)$ samples from the value
% distribution suffice for the the descending auction run on the empirical
% distribution to have the same set of approximate equilibria as the first price
% auction without search cost under the empirical distribution transformed \`a la
% \citet{KWW16}.

This model was proposed and studied by \citet{KWW16},
who showed that a \emph{descending price auction}, absent strategic considerations, implements the optimal algorithm for maximizing the auction's efficiency, and that 
there is a bijection (preserving allocation and payments) between the equilibria of a descending price auction with search costs and the equilibria
of a first price auction
without search costs but with the value distributions transformed.
Using this transformation, they conclude that even when the bidders strategize over their bids, the descending auction's efficiency is near optimal.

However, both the bijection of equilibria and the transformation of distributions are distribution-dependant. The main result of this section is that, given search costs and samples from unknown value distributions, $\tilde O(n / \eps^2)$ samples 
suffice to construct a mapping and a transformation, such that any equilibrium of the first price
auction without search costs under the transformed empirical distribution can be mapped to an approximate equilibrium of the descending auction run on the true
distribution.

%In an auction with search cost, the maximum
%welfare under the transformed distribution is just the maximum welfare
%achievable under the original distributions with search costs.

The reduction from auctions with search costs to auctions without search costs is closely related to the Pandora's Box algorithm
\citep{Weitzman79}. This algorithm maximizes the social welfare of an auction when there is search cost. 
The sample complexity of the algorithm is interesting in its own right.
We improve an upper bound on its sample complexity given recently by \citet{GHTZ19}
in Section~\ref{sec:pandora}. Then in Section~\ref{sec:fpa-pandora} we combine the key idea of Pandora's Box algorithm with results
from Section~\ref{sec:fpa} to obtain a sample complexity bound for
\citeauthor{KWW16}'s reduction.


% We first review the algorithm, known as the Pandora's Box algorithm
% \citep{Weitzman79}, for
% maximizing the welfare when there is search cost. 
% The sample complexity of the algorithm is interesting in its own right.
% We improve an upper bound on its sample complexity given recently by \citet{GHTZ19}
% in Section~\ref{sec:pandora}.  
% Then in Section~\ref{sec:fpa-pandora} we combine the key idea of Pandora's Box algorithm with results
% from Section~\ref{sec:fpa} to obtain a sample complexity bound for
% \citeauthor{KWW16}'s reduction.


